Model-Predictive Control of Blood Suction for Surgical Hemostasis using Differentiable Fluid Simulations

Recent developments in surgical robotics have led to new advancements in the automation of surgical sub-tasks such as suturing, soft tissue manipulation, tissue tensioning and cutting. However, integration of dynamics to optimize these control policies for the variety of scenes encountered in surgery remains unsolved. Towards this effort, we investigate the integration of differentiable fluid dynamics to optimizing a suction tool's trajectory to clear the surgical field from blood as fast as possible. The fully differentiable fluid dynamics is integrated with a novel suction model for effective model predictive control of the tool. The differentiability of the fluid model is crucial because we utilize the gradients of the fluid states with respect to the suction tool position to optimize the trajectory. Through a series of experiments, we demonstrate how, by incorporating fluid models, the trajectories generated by our method can perform as good as or better than handcrafted human-intuitive suction policies. We also show that our method is adaptable and can work in different cavity conditions while using a single handcrafted strategy fails.

==> MPC Fluid Suction ICRA/sections/abstract.tex <==
Recent developments in surgical robotics have led to new advancements in the automation of surgical sub-tasks such as suturing, soft tissue manipulation, tissue tensioning and cutting.
% However, no work has been done to incorporate fluid dynamics modeling with surgical robotics.
However, integration of dynamics to optimize these control policies for the variety of scenes encountered in surgery remains unsolved.
Towards this effort, we investigate the integration of differentiable fluid dynamics to optimizing a suction tool's trajectory to clear the surgical field from blood as fast as possible.
The fully differentiable fluid dynamics is integrated with a novel suction model for effective model predictive control of the tool.
The differentiability of the fluid model is crucial because we utilize the gradients of the fluid states with respect to the suction tool position to optimize the trajectory.
% In this paper we present a method for fluid control in a surgical scenario utilizing differentiable fluid simulation in a model predictive framework.
% We apply it to the surgical sub-task of blood suction.
Through a series of experiments, we demonstrate how, by incorporating fluid models, the trajectories generated by our method can perform as good as or better than handcrafted human-intuitive suction policies.
We also show that our method is adaptable and can work in different cavity conditions while using a single handcrafted strategy fails. 

% Furthermore, we perform open-loop control experiments on the  da  Vinci  Research Kit (dVRK) robot for validation. The results show that trajectories generated from our method are robust enough for sim-to-real autonomous blood suction applications.

% naive solutions such as simply suction at the center of the blood volume do not take into account the physics of the fluid and the geometry of the cavity. On the other hand, a human-intuitive strategy of suctioning against the flow of the blood will fail when the flow splits into multiple direction. 

% In this work we present a method for controlling suction utilizing a diffrentiable fluid simulation in a model predictive framework. Through a series of simulated experiments, we show that our method can perform just as well or better than handcrafted human-intuitive suction strategies in terms of how well the cavity is cleared and how fast it is achieved. 

% We also show that our method is adaptable and can work in different cavity conditions when using a single handcrafted strategy fails. Furthermore, the open-loop control experiments  have  been  conducted  on  the  da  Vinci  ResearchKit  (dVRK)  robot  for  validation.  The  results  show  that  our solution  is  robust  enough  for  sim-to-real  autonomous  blood suction  applications

==> MPC Fluid Suction ICRA/sections/discussion_and_conclusion.tex <==
In this work we presented a method for incorporating differentiable fluid modeling into autonomous surgical robotics. We applied this method to the surgical sub-task of controlling suction to clear the surgical field of blood during a hemorrhage.
The gradients from the PBF model were used in an MPC framework. The resulting real-world trajectories lead to low percentages of remaining blood despite differences in the fluid parameters between the real and simulated scenes such as surface tension and adhesion of the fluid, and suction strength.
To better overcome these sim-to-real challenges, we plan to integrate visual feedback to initialize and correct the PBF model in real-time using our recently developed blood tracking algorithm \cite{richter2020autonomous}. Finally, our method can be generalized to incorporate different physics models into automating surgical tasks.
% The back-propagation approach of differentiation can be applied to almost any series of computations.
Gradients can be derived for not only fluid models, but also for rigid and soft body interactions by viewing their operations as computational graphs in a unified framework \cite{macklin2014unified}.

%For future work, we will investigate similar differentiable dynamics such that surgical task automation can plan for interactions between rigid bodies, soft tissue, and fluids in a cohesive framework \cite{richter2019open}.

% In this work we present a method for incorporating fluid modeling into autonomous surgical robotics. We apply this method to the surgical sub-task of controlling suction to achieve hemostasis during surgeries. Our proposed method utilizes position-based fluid simulation made differentiable using back-propagation. The gradients from this simulation are used in a model predictive control framework to clear the surgical cavity of blood as fast as possible. Through a series of simulated experiments, we see that different cavity and emission conditions require different suction strategies to clear the blood effectively. Because of this, simply picking one strategy such as fixing the suction tool at the emission point or follow an end-to-emit trajectory for all cases will not lead to the most optimal suction results. With these experiments, we show how our method can generate suction trajectories that perform at the same level or better than the handcrafted strategies. This shows that our method is adaptable and can be effective in many different cavity conditions while using a single controls formulation. This is possible because our method takes into account the physics of the blood and cavity implicitly, without needing to reference explicit human-crafted strategies.

% From the experiments with the silicon rubber cavity, we see that, for this particular cavity geometry, suction should start in the middle area for good performance in the early stage. Our method generates trajectories that have this characteristic and results in fast suction in the early and middle stages. Furthermore, our trajectories also lead to low percentages of remaining blood despite differences in the fluid parameters such as surface tension and adhesion to cavity surfaces between the real and simulated scenes. A natural extension of this work is to make the fluid simulation more realistic by incorporating characteristics such as adhesion, cohesion, viscosity, etc, so that these factors can be accounted for in the trajectory optimization process.

% For future work we want to extend the improvements 

% Gradients can be easily derived for not only fluid models, but rigid body and soft tissue interactions as well by viewing their operations as computational graphs. Recent advancements in physics simulations such as \cite{macklin2014unified} have created unified solvers that can handle rigid bodies, deformable objects, as well as fluids all in the same framework.
% This means it is possible to back-propagate and differentiate through a model that includes diverse object types. This also means we can use similar controls formulations and optimization techniques to automate surgical tasks that involve interactions between physical objects in different states, which is the case in almost all realistic scenarios. 


==> MPC Fluid Suction ICRA/sections/experiments.tex <==
% To evaluate the proposed control algorithm, we perform experiments in simulation.
% We compare the performance of our algorithm to naive approaches such as fixed point suction, as well as handcrafted trajectories.
% We also conduct a lab experiment to validate that the trajectories generated using our method are effective for real world use.
The efficiency of the proposed suction control algorithm is tested in both simulated scenes and a real world example.
Performance is evaluated by measuring how quickly the fluid is removed.
It is also compared against hand-crafted trajectories to highlight the generalizability of the proposed methods to different scenarios.

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.15\textwidth}
        \includegraphics[width=1.0\textwidth]{figures/cavity1_real_anno.png}
        \label{fig:cavity1_real}
    \end{subfigure}
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figures/cavity1_sim_anno.png}
        \label{fig:cavity1_sim}
    \end{subfigure}
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figures/cavity3_sim_anno.png}
        \label{fig:cavity3_sim}
    \end{subfigure}
    \caption{Comparison between a real surgical cavity and our simulated cavity. \textbf{Left:} the scene of a thyroidectomy conducted on a pig, where a rupture occurred on the carotid artery. \textbf{Middle:} a simulated cavity that has the same general flow pattern as the real scene, denoted as \textit{case 1}. \textbf{Right:} same cavity but with a different blood emission point, denoted as \textit{case 2}. The green paths and arrows denote the general direction of blood flow. }
    \label{fig:cavity_side_by_side}
\end{figure}

\begin{figure}[t]
    \centering
    \vspace{1.8mm}
    \begin{subfigure}{0.235\textwidth}
        \centering
        \includegraphics[trim=0cm 0cm 0cm 0cm, clip,width=1.0\textwidth]{figures/sim_suction_plot_case1.pdf}
        \label{fig:sim_suction_curve_case1}
    \end{subfigure}
    \begin{subfigure}{0.235\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figures/sim_suction_plot_case2.pdf}
        \label{fig:sim_suction_curve_case2}
    \end{subfigure}
    \caption{Suction curves for the simulated scenes normalized by initial volume. The time axis starts at 200 because of the warm-up period for filling the cavity. \textbf{Left:} In \textit{case 1}, both our method and the end-to-emit trajectory can reach an equilibrium where the cavity is mostly clear, with out method being much faster. \textbf{Right:} In \textit{case 2}, the fastest method are our method and suctioning at the emission point.}
    \label{fig:sim_suction_curves}
\end{figure}


\subsection{Simulated suction experiments}

Two simulated scenes used to evaluate the proposed control strategy are shown in Fig. \ref{fig:cavity_side_by_side}. These scenes are motivated by real surgical cases where a surgeon error in a live thyroidectomy caused bleeding to occur. A simulation was built to mimic this scenario, with different blood emission locations. The simulation used a time step of $\Delta_t = 0.01$s, the maximum number of particles was limited to $N=2000$, and 200 simulation steps were taken before the robot can take its first action.
The MPC controller used a horizon $h=10$, and the initial suction point selection uses a look-ahead window of $m=100$.
% used a look-ahead value of $m=100$ and $h=10$ for initialization and normal control respectively, 
A total of 10 samples were used for initial point selection.
The target height was set to $y_{goal} = 10$cm, suction strength $\mathcal{K} = 100 $, $\sigma_x = \sigma_z = \sqrt{0.5}$.
The maximum change in end-effector position was also limited to 0.5mm every step to be realistic.
Finally, the gradients used a learning rate of 0.1 with normalized gradients such that their components have a maximum magnitude of 1.

% We create cavities with simplified geometries that aim to emulate the general flow pattern of a real cavity. The two cases we use in our experiments are shown in Figure \ref{fig:cavity_side_by_side}. 

% To simulate how our MPC algorithm would work in the real world, we use three separate fluid simulations. The \textit{real world} represents the surgical environment that we are attempting to control. Like in the real world, we can only obtain the past and present states of this simulation. %since we can not have information about the future in a real world scenario. 
% At each timestep, particle positions and velocities are extracted from the \textit{real world}, which emulates the perception process.

% The \textit{main sim} represents the internal model in our MPC algorithm. This simulation runs for the MPC horizon $h=10$ steps, and its states are used to compute the loss and gradients. The optimal control action is obtained using a descent method on the gradients of the \textit{main sim}. 
% %For every iteration of gradient descent, this simulation is reset and reinitialized with the particle states extracted from the \textit{real world}.

% For selection of the initial suction point, we use the \textit{auxiliary sim} which runs for the look-ahead window $m=100$ steps. It is initialized using the \textit{real world} states, and the initial suction point is taken from sampled \textit{real world} particle positions. The  number of remaining particles after $m$ steps is used to determine the best initial suction point. 

% In our experiments, the simulation step size is $\Delta t=0.01s$. There is a $200$-step warm-up period for the blood to fill the cavity before suction control is engaged. Blood particles are continuously emitted into the cavity until the end of the simulation. The target height used in the loss function is $y_{goal}=10cm$. For gradient descent, we use a learning rate of $0.1$, with normalized gradients such that their components have a maximum magnitude of $1$. We also limit the change in end effector position between each step to be less than $0.5mm$. All suction policies are simulated with the same parameters.

Four hand-crafted control policies for controlling the suction nozzle were also developed to compare against the proposed MPC method.
They are: 1) \textit{Fixed emission}: stays at the emission point 2) \textit{Fixed end}: stays at the end point where the fluid could flow too 3) \textit{Fixed middle}: stays at the middle of the fluid flow 4) \textit{End-to-emit}: moves from the end to emission point at a constant rate.
% \begin{enumerate}
%     \item \textit{Fixed emission}: stays at the emission point
%     \item \textit{Fixed end}: stays at the end point where the fluid could flow too
%     \item \textit{Fixed middle}: stays at the middle of the fluid flow
%     \item \textit{End-to-emit}: moves from the end to emission point at a constant rate
% \end{enumerate}
To evaluate the performance of the methods, curves were generated by plotting the amount of remaining blood (normalized by the initial volume) against time (in simulation timesteps).
Good suction performance should have little blood at the end of the simulation.
% Recall that excess blood in the surgical cavity can impede the field of view and negatively affect later actions for hemostasis. 
% So another metric is the area under the suction curve (AUC), which can be interpreted as the total penalty, over time, for blood blocking the field of view. Since this is a penalty, we want it to be as low as possible.
Another metric was the time it takes to reduce the amount of blood in the cavity by 50\% and 90\%, computed as
\begin{equation}
\begin{aligned}
        \tau_{50\%} = \; & \text{min} & & t-t_0 \\
                      & \text{s.t.} & & f(t) <= 50\%
\end{aligned}
\label{eq:convergence_time}
\end{equation}
where $f(t)$ is the suction curve as a function of time, $t_0$ is the time at which suction begins, and $t_f$ is the time at which the simulation ends. The time for 90\% reduction was computed similarly. Note that the percent reduction time only makes sense if the suction policy actually reduced the amount of blood by the targeted amount. Otherwise the percent reduction time was not computed.

\begin{table}[t]
    \centering
    \vspace{1.8mm}
    \begin{tabular}{cccccc}
         \hline
         & Our & Fixed:  & Fixed:  & Fixed:  & End-to-emit\\
         & method & emission & end & middle & trajectory\\
         \hline
        %  Final & & & & & \\
         Residual & 5.5\% & 28.0\% & 64.5\% & 27.0\% & \textbf{2.5}\% \\
        %  & 11 & 56 & 129 & 54 & \textbf{5} \\ 
         %AUC & 122.73 & 264.98 & 432.08 & 202.80 & 219.38 \\
         $\tau_{50\%}$ & \textbf{36} & 87 & -- & 23 & 90 \\
         $\tau_{90\%}$ & \textbf{162} & -- & -- & -- & 255 \\
         \hline
    \end{tabular}
    \caption{Residual of blood after trajectory is executed and percent reduction time for \textit{case 1}.
    %Final count is measured in number of particles, while the convergence times are measured in simulation time steps. Our method achieves similar final particle count as the end-to-emit trajectory, while having significantly lower convergence time, which shows that our method suctions much faster.
    }
    \vspace{-3mm}
    \label{tab:results_case1}
\end{table}

\begin{table}[t]
    \centering
    \begin{tabular}{ccccc}
         \hline
         & Our & Fixed:  & Fixed:  & End-to-emit \\
         & method & emission & end (avg) & trajectory (avg)\\
         \hline
        %  Final & & & & \\
         Residual & \textbf{1.5}\% & 2.0\% & 65.0\% & 3.8\% \\
        %  Final count & \textbf{3} & 4 & 130 & 7.5 \\ 
         %AUC & 76.04 & 82.85 & 424.81 & 185.33 \\
         $\tau_{50\%}$ & 21 & \textbf{18} & -- & 87.5 \\
         $\tau_{90\%}$ & \textbf{102} & \textbf{102} & -- & 172.5 \\
         \hline
    \end{tabular}
    \caption{Residual of blood after trajectory is executed and percent reduction time for \textit{case 2}.
    % Final count is measured in number of particles, while the convergence times are measured in simulation time steps. Because the scene is roughly symmetric, we take average of policies that have left and right versions. Here we see that our method, fixed suction at the emission point, and the end-to-emit trajectory can all achieve a very low final particle count. The suction speed of our method is comparable to fixed at emission point, which is the fastest.
    }
    \label{tab:results_case2}
\end{table}

The results from the experiments are shown in Fig. \ref{fig:sim_suction_curves} and Table \ref{tab:results_case1} and \ref{tab:results_case2}.
As is evident by the results, the proposed method performed as good as, if not better than, the best hand-crafted policies.
In \textit{case 1}, the blood flowed around the obstacle from right to left, hence making the best hand-crafted policy, end-to-emit trajectory, slow but complete in suctioning the blood.
However, in \textit{case 2} this end-to-emit strategy failed since the blood emits closer to the middle of the cavity hence diverting in two directions.
Meanwhile the opposite behavior occurred for the fixed emission control, where it failed in \textit{case 1} but was the best strategy in \textit{case 2}. This means the hand-crafted policies had limited success only in a single scenario the proposed method successfully generalized to both cases.

% .... 

To better understand the adaptability of the proposed method to different emission scenarios, it was tested on a large variety of emission points in the same cavity.
The emission points were evenly spaced along the sides of the cavity, with emission directions normal to the walls, hence pointing towards the inside of the cavity.
The lengths of the resulting trajectories as well as suction speed measured by 60\% convergence time are plotted as heatmaps in Fig. \ref{fig:heatmap}.
Typically the trajectories for emission points near the middle of the cavity will be shorter as the suction tool will stay near emission.
Meanwhile for emission points near the top left or right corners, the trajectory will follow more similarly to a long, end-to-emit-type path.

% From these two cases, we see that our method can adapt and generate very different trajectories depending on the location of the emission point.
% To gain insight into how the trajectory varies as we change the emission location, we test our method on the same cavity with different emission points.
% The emission points are evenly spaced along the sides of the cavity, with emission directions normal to the walls, pointing inside the cavity.
% The lengths of the resulting trajectories as well as suction speed measured as the 60\% convergence time are plotted as heatmaps, shown in Fig. \ref{fig:heatmap}.
% From the left plot, we see that in general, for emission points near the middle of the cavity, our method will take very short trajectories, which means it stays near the middle.
% For emission points near the top left and top right corners of the cavity, our method will follow an end-to-emit type path, with a longer trajectory length.
% From the right plot, we see the intuitive result where longer trajectories typically lead to larger 60\% convergence time, which means suction is slower. 

\begin{figure}[t]
    \centering
    \vspace{1.8mm}
    \begin{subfigure}{0.205\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figures/traj_length_heatmap.pdf}
    \end{subfigure}%
    \begin{subfigure}{0.226\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figures/final_percent_heatmap.pdf}
    \end{subfigure}
    \caption{Applying our method to different emission points in the cavity. The locations of the tiles represent the locations of the emission points, while the colors denote trajectory length in $cm$ (left) and normalized amount of residual blood (right). While the trajectories vary in length as the emission point changes, they generally achieve low residuals. This demonstrates how MPC is able to adapt to different emission scenarios.
    % The trajectories generated by our method is longer when the emission point is near the top left or top right corner of the cavity, and shorter when the emission point is near the middle. 
    % \textbf{Right:} Longer trajectories are correlated with larger 60\% convergence time, which means suction is slower.
    }
    \label{fig:heatmap}
    \vspace{-1.8mm}
\end{figure}


\subsection{Trajectory validation}

% In order to validate the suction trajectories generated using our algorithm, we repeat the simulation experiments in a cavity made out of silicone rubber. Water with red dye is used to emulate blood flow, which is manually injected into the cavity with a syringe. The da Vinci PSM arm is used to control a EndoWrist Suction/Irrigator tool for suctioning. When testing our method, the suction tool follows the generated trajectory in an open-loop fashion. Color segmentation on images of the cavity is used to estimate the amount of blood in the cavity. We use thresholding in the HSV color space to detect pixels of blood. The area covered by the blood pixels and a calibrated depth curve in HSV space is used to estimate the volume of blood at each image frame. Finally, for each suction policy, we perform 3 trials and average the results to reduce the effects of human errors such as inconsistent manual injection speed. In each trial, the cavity is pre-filled with blood, and more blood is continuously injected when suction starts to emulate the conditions in the simulated experiments.

In order to validate the suction trajectories generated using our algorithm, we repeated the simulation experiments in a cavity made out of silicone rubber. 
Water with red dye was used to emulate blood flow, which was manually injected into the cavity with a syringe similar to the previously described \textit{case 1} and \textit{case 2} simulated scenes.
A Patient Side Manipulator (PSM) from the dVRK \cite{kazanzides2014open} was fitted with a EndoWrist Suction/Irrigator tool for suctioning.
The cavity and PSM arm were converted into a unified camera frame defined by dVRK's stereo endoscope so that trajectories could be defined in a common reference frame.
To register the cavity, an Aruco marker was attached to it and the pose was solved for using the Aruco library \cite{garrido2014automatic}.
Meanwhile the end-effector of the suction tool was localized in camera frame using our previously developed work, SuPer \cite{li2020super}.


\begin{figure*}[t!]
    \centering
    \vspace{1.8mm}
%     \begin{subfigure}{0.105\textwidth}
% 	\includegraphics[width=1.0\textwidth]{figures/case1_ours/sim_case1_our_trajectory.pdf}
% 	\end{subfigure}
    \begin{subfigure}{0.195\textwidth}
	\includegraphics[width=1.0\textwidth]{figures/case1_ours/render_102.pdf}
	\end{subfigure}
    \begin{subfigure}{0.195\textwidth}
	\includegraphics[width=1.0\textwidth]{figures/case1_ours/render_146.pdf}
	\end{subfigure}
	\begin{subfigure}{0.195\textwidth}
	\includegraphics[width=1.0\textwidth]{figures/case1_ours/render_173.pdf}
	\end{subfigure}
	\begin{subfigure}{0.195\textwidth}
	\includegraphics[width=1.0\textwidth]{figures/case1_ours/render_200.pdf}
	\end{subfigure} 
	\begin{subfigure}{0.195\textwidth}
	\includegraphics[width=1.0\textwidth]{figures/case1_ours/render_399.pdf}
	\end{subfigure}
	
% 	\vspace{-0.5mm}
    \vspace{1mm}
	
% 	\begin{subfigure}{0.105\textwidth}
% 	\includegraphics[width=1.0\textwidth]{figures/case1_ours/real_case1_our_trajectory.pdf}
% 	\end{subfigure}
	\begin{subfigure}{0.195\textwidth}
	\includegraphics[width=1.0\textwidth]{figures/case1_ours/image-018-crop.jpeg}
	\end{subfigure}
    \begin{subfigure}{0.195\textwidth}
	\includegraphics[width=1.0\textwidth]{figures/case1_ours/image-020-crop.jpeg}
	\end{subfigure}
	\begin{subfigure}{0.195\textwidth}
	\includegraphics[width=1.0\textwidth]{figures/case1_ours/image-022-crop.jpeg}
	\end{subfigure}
	\begin{subfigure}{0.195\textwidth}
	\includegraphics[width=1.0\textwidth]{figures/case1_ours/image-026-crop.jpeg}
	\end{subfigure} 
	\begin{subfigure}{0.195\textwidth}
	\includegraphics[width=1.0\textwidth]{figures/case1_ours/image-042-crop.jpeg}
	\end{subfigure}
	
    \caption{Comparison between the simulated scene (top) and experiments with the real cavity (bottom) for \textit{case 1} using our method.
    % In both cases majority of the blood is successfully removed.
    Unexpected residual blood occurs in the real world due to unaccounted factors such as surface tension and adhesion.
    Nonetheless, it still effectively removed more than 90\% of the injected blood.
    % The first image in each row shows the trajectory followed by the tool, with the green arrow denoting the blood emission point.
    % In the simulation, our trajectory reaches an equilibrium where the cavity is almost completely clear. While the trajectory followed by the suction tool closely matches our simulation, due to factors such as surface tension and adhesion, a thin layer of blood remains at the end of the real experiment. However, the completion of suction can be confirmed with the amount of blood remaining less than 10\% of the initial volume.
    }
    % \vspace{-1.8mm}
    \label{fig:case1_sim_real_comparison}
    
\end{figure*}



Since trajectories are now required to be described in the common camera frame, the suction tool trajectories, defined in the model's coordinate frame, needs to be properly transformed into the camera frame. This is done by setting the position of the end-effector (suction nozzle) in the PSM base frame, $\mathbf{b}_{t}$, to:
\begin{equation}
    \overline{\mathbf{b}}_{t+1} = \begin{cases} \gamma_s \frac{\mathbf{d}_{t}}{||\mathbf{d}_{t}||} + \overline{\mathbf{b}}_{t}   & \text{if } \mathbf{d}_{t} > \gamma_s\\
    \mathbf{d}_{t} + \overline{\mathbf{b}}_{t} & \text{if } \mathbf{d}_{t} \leq \gamma_s
    \end{cases}
\end{equation}
where $\gamma_s = 0.75$mm is the max step size, the operator $\overline{\cdot} = \begin{bmatrix} \cdot& 1\end{bmatrix}^\top$ gives the homogeneous representation of a point, and the direction, $\mathbf{d}_t$, was computed as
\begin{equation}
    \mathbf{d}_t = \mathbf{T}^b_c \overline{\mathbf{x}}_{e,t} - \overline{\mathbf{b}}_{t}
\end{equation}
with $\mathbf{T}^b_c \in SE(3)$ is the camera to base transform estimated in real-time \cite{li2020super} and $\mathbf{x}_{e,t}$ was the control action defined by the MPC controller.
%The orientation of the end-effector was simply set to always be in the direction of gravity.
Inverse kinematics was then used to convert the position, $\mathbf{b}_t$, and orientation to joint angles which were regulated by the robot.

% The da Vinci PSM arm is used to control a EndoWrist Suction/Irrigator tool for suctioning. When testing our method, the suction tool follows the generated trajectory in an open-loop fashion.
% Color segmentation on images of the cavity was used to estimate the amount of blood in the cavity.
The amount of blood in the cavity was estimated using images from the dVRK's stereo endoscope.
Color segmentation to detect the blood was done by manually setting thresholds in the hue, saturation, value (HSV) color space.
% We use thresholding in the HSV color space to detect pixels of blood.
We assume that the concentration of red dye in the water was uniform, which means the attenuation of light through the fluid is proportional to depth by the Beer-Lambert Law \cite{ingle1988spectrochemical}. 
Calibration was performed by taking images of the cavity filled with different volumes of blood and fitting a relationship between the depth of blood and the pixel values in each of the three channels.
The area covered by the blood pixels and the calibrated depth curve in HSV space are used to estimate the volume of blood at each image frame. This model is a simple approximation of the volume of blood, which can only be truly known if one observed the underlying tissue topology before being filled with blood. Naturally, MPC's iterative approach continuously corrects for this volume assumption as more of the tissue topology is revealed, so this first-order approximation is reasonable.
% Finally, for each suction policy, three trials were performed, and the results averaged, to reduce the effects of human errors such as inconsistent manual injection speed.

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figures/real_suction_plot_case1.pdf}
    \end{subfigure}
    \vspace{-2mm}
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figures/real_suction_plot_case2.pdf}
    \end{subfigure}
    \caption{
    From top to bottom, the plots show suction results from real world experiments for \textit{case 1} and \textit{case 2} respectively, normalized by the initial volume.
    The proposed method reacts more efficiently as seen by the lack of bump at $(b)$, reaches the linear decrease faster at $(c)$, and typically removes the most blood at the end $(d)$.
    % Suction curves for experiments with a silicone rubber cavity. We analyze the curves by splitting them into 4 distinct stages: $(a)$ system initialization; $(b)$ early stage; $(c)$ middle stage; $(d)$ end stage. The top plot corresponds to experiments for \textit{case 1}, and the bottom plot corresponds to experiments for \textit{case 2}.
    }
    \label{fig:real_suction_curve}
\end{figure}


Three trials were repeated per policy and the results are averaged.
In each trial, the cavity was pre-filled with blood, and more blood was continuously injected when suction started to emulate the conditions in the simulated experiments.
The suction curves for experiments with the silicone rubber cavity are shown in Figure \ref{fig:real_suction_curve}. We analyze the suction curves by roughly splitting each trial into 4 distinct stages: $(a)$ where the tool moved to initial position without suctioning $(b)$ when suction and injection began $(c)$ where suction engaged  with the blood for the same time; $(d)$ where suction and injection had been engaged for a long time and the tool reaches the end of the trajectory.

% In stage $(a)$, since there is no suction, the behavior is the same for all suction policies. 

In stage $(b)$, the amount of blood increased as suction started for most of the hand-crafted policies. This means the rate of suction was slower than the rate of blood injection.
Meanwhile the proposed method was able to consistently circumvent this, hence being more efficient.
% We find that for suction policies that have an initial increase of remaining blood, the suction tool is at the top left or top right corner of the cavity during stage $(b)$, while policies that do not see this behavior start in the middle of the cavity. 
In stage $(c)$, suction and injection reached an equilibrium where the percentage of remaining blood decreased at a steady rate. 
This rate of decrease was seen to be roughly constant for all policies. 
However, the proposed method was able to reach this state faster due to being more efficient in stage $(b)$.
% In this state, the percentage reaches similar rates of decrease for different suction policies within the same case.

A discrepancy between the simulation-and-real world was seen at stage $(d)$ where in the real world a thin remaining layer of blood is left over.
An example for \textit{case 1} is shown in Figure \ref{fig:case1_sim_real_comparison}.
In the simulation, the blood particles was able to flow without sticking to the face of the cavity, while a patch of blood was stuck in the left half of the cavity in the real experiment due to surface adhesion.
Nonetheless, our method still results in a low percentage of remaining blood at the end of the task.

% In stage $(d)$, most of the blood in the cavity have been cleared. The remaining blood in the cavity is typically a thin layer, which causes the effects of surface tension and adhesion to be more pronounced.
% An example for \textit{case 1} is shown in Figure \ref{fig:case1_sim_real_comparison}.
% In the simulation, the blood particles can flow without sticking to the face of the cavity, while a patch of blood is stuck in the left half of the cavity in the real experiment.
% Thus, it might be necessary to back track to previously suctioned areas in order to completely clear the cavity.

% Considering the characteristics across these 4 distinct stages, the trajectories generated with the our method typically start in the middle area of the cavity, which leads to good behaviors in the early stage where the percentage of remaining blood does not increase beyond the initial value. This also helps to reduce the duration of the early stage, which means faster suction compared to other policies. Finally, our trajectories also lead to a low percentage of remaining blood in the end stage.


==> MPC Fluid Suction ICRA/sections/introduction.tex <==
Automating robotic surgeries has generated considerable interest in the robotics research community \cite{yipDasJournal} given the development of commercially available surgical robotic systems like the da Vinci Surgical System and open-source platforms such as the da Vinci Research Tool Kit (dVRK) \cite{kazanzides2014open}, Some important goals of surgical automation research are to develop algorithms and systems that can leverage the precision of robots to improve the safety of operations, reduce surgeon fatigue by taking over repetitive tasks, and improve access to surgical care for communities where clinician availability is lacking. Initial research has been done towards automating surgical sub-tasks such as soft tissue manipulation \cite{Shin_2019,attanasio2020autonomous}, tensioning and cutting \cite{thananjeyan2017multilateral,le2018semi}, suturing \cite{zhong2019dual, shademan2016supervised, pedram2017autonomous}, and debridement removal \cite{richter2019open, pedram2019toward}.

% However, previous surgical task automation efforts often make assumptions about the environment dynamics and its interaction with the surgical tools.
% While these assumptions provide good initial results, they must be eventually lifted to develop more generalizable autonomous control policies.
An important component to  automating of surgical tasks is understanding the interaction of the surgical tool and the environment.
Modelling the interaction between surgical tools and the environment has previously been done using data driven approaches in the form of reinforcement learning \cite{thananjeyan2017multilateral} and learning from demonstration \cite{murali2015learning}.
While these methods provide good initial results, the policies produced are limited by the variation in the scenarios in which the policy is trained upon, and those policies may fail in new environments. 
In order to develop more generalizable autonomous control policies, an online model-predictive approach is preferred. we consider differentiable dynamics where gradients can be computed through the predictive models, hence allowing for trajectories to be efficiently optimized on a per-scenario basis.
This allows the robot to adapt its trajectories, in real-time, to the constantly deforming and highly variable surgical environment.
Such differential dynamics models have been demonstrated in \cite{ummenhofer2019lagrangian}. \cite{li2018learning}, and \cite{schenck2018spnets}, but have not been applied to surgical robotics.

% Recently, outside the surgical robotics community, there have been demonstrations of successful differentiable dynamic models such as \cite{ummenhofer2019lagrangian}. \cite{li2018learning}, and \cite{schenck2018spnets}.
% By being natively differentiable, gradients can be computed through the predictive models, allowing for trajectories to be efficiently optimized on a per-scenario basis.
% This allows the robot to adapt its trajectories, in real-time, to the constantly deforming and highly variable surgical environment.

% In this paper we demonstrate how fluid modeling can be incorporated into autonomous surgical robotics, focusing on the surgical sub-task of blood suction, which is an important technique for achieving hemostasis when hemorrhage occurs during an operation. A typical scenario will involve 4 steps. First, blood is suctioned to clear the cavity. Then the ruptured vessel is identified, and pinching is used to temporarily stop the bleeding. Finally, the vessel is sealed using a ligation clip. Among these steps, the suctioning blood as quickly as possible is critical to achieving hemostasis because excess fluid in the surgical cavity decreases the field of vision, which will prevent the surgeon from identifying the vessel and sealing it in a timely manner. 
% An autonomous surgical robot can be beneficial to this process if it can control suction with real-time and predicable motion. 

\begin{figure}
    \centering
    \vspace{1.8mm}
    \begin{subfigure}{0.47\textwidth}
        \includegraphics[width=1.0\textwidth]{figures/case2_tool_motion_real.pdf}
        \label{fig:case2_tool_motion_real}
    \end{subfigure}
    % \begin{subfigure}{0.25\textwidth}
    %     \includegraphics[width=1.0\textwidth]{figures/case2_trajectory.pdf}
    %     \label{fig:case2_trajectory}
    % \end{subfigure}
    
    % \caption{Our suction control algorithm in action. \textbf{Top:} A suction trajectory generated using our model predictive control algorithm being deployed in a silicon rubber cavity. \textbf{Bottom:} A comparison between the desired trajectory generated by our method and the actual trajectory executed by the dVRK robot. By implicitly incorporating fluid dynamics with gradients back-propagated through a position-based fluid simulation, our method generated a trajectory that moves around the emission point, then stays near it to suction the continuously emitted blood to keep the cavity as clear as possible.}
    \caption{A suction trajectory generated using our model predictive control algorithm being deployed in a silicon rubber cavity. By explicitly incorporating fluid dynamics with gradients back-propagated through a position-based fluid simulation, our method is able to efficiently optimize trajectories to rapidly clear the surgical field from blood in a model-predictive manner.
    % our method generates a trajectory that moves around the emission point, then stays near it to suction the continuously emitted blood to keep the cavity as clear as possible.
    }
    \label{fig:case2_real_motion_and_trajectory}
\end{figure}

% An obvious control policy for suction might be to simply place the nozzle wherever blood is detected. However, this policy does not consider the geometry of the surgical cavity nor the fluid dynamics model of the blood flow, which can increase the time it takes to clear the cavity. 



% In this work, we develop a control method that incorporates the physics of the surgical scene in order to clear the cavity of blood as quickly as possible. To this end, we present the following contributions:
In this work we will investigate integration of differentiable dynamics from the perspective of fluids and autonomous suctioning.
Suctioning is the first essential step to achieving hemostasis, which is the process of suctioning blood, finding the bleed, and closing a ruptured vessel during a surgery.
Ruptured vessels can occur at any moment and require an immediate reaction.
By clearing the surgical field from blood in an quick manner, a surgeon can identify the rupture vessel and close it effectively.
% This paper, to the best of our knowledge, presents the first work to consider fluid control in autonomous surgery. 
To accomplish this, we develop a model-predictive control (MPC) strategy utilizing differentiable blood fluid dynamics for the surgical scene.  Specifically, we present the following contributions:
\begin{enumerate}
    \item an end-to-end differentiable position-based blood fluid simulation,
    \item a differentiable model of suction that can be embedded into the fluid simulation, and
    \item a model-predictive control algorithm that incorporates blood fluid dynamics in autonomous surgical robotics.
\end{enumerate}
Using a natively differentiable fluid model provides a robust method for integrating the behavior of flowing blood into an optimization framework. We study and evaluate the proposed method through simulated experiments to highlight the advantages and generalizability of the resulting control policy for blood suction.
We also provide an implementation of the method on the da Vinci Research Kit (dVRK) \cite{kazanzides2014open} to show the real-world effectiveness of the proposed methods.


% To the best of our knowledge, there is no prior work on incorporating blood fluid dynamics into the task of suction control in the field of autonomous surgical robotics. In this work, we develop a control method utilizing blood fluid simulation to take into account the physics of the surgical scene when optimizing the suction trajectory. To this end, we present the following contributions:
% \begin{enumerate}
%     \item an end-to-end differentiable position-based blood fluid simulation,
%     \item a differentiable model of suction that can be embedded into the fluid simulation, and
%     \item a model predictive control algorithm that incorporates blood fluid dynamics in autonomous surgical robotics.
% \end{enumerate}
% \textcolor{red}{Add closing sentences here which summarize the experiments from a high level (implemented on dVRK to show real world effectiveness)}

==> MPC Fluid Suction ICRA/sections/methods.tex <==

\begin{algorithm}[t]
\SetAlgoLined

$\mathbf{v}_i = \mathbf{v}_i + \Delta t f_{ext}(\mathbf{x}_i)$ \Comment{{\scriptsize apply external forces}} \\
$\mathbf{x}_i^* = \mathbf{x}_i + \Delta t \mathbf{v}_i$ \Comment{{\scriptsize predict position}} \\
$\mathbf{n}_i \leftarrow \mathrm{FindNeighboringParticles}(\mathbf{x}_i^*)$  \\

% \Comment{constraint solving step} \\
\While{iter $<$ SolverIterations}{
% \For{constraint $C \in M$}{
% \For{particle $i \in N$}{
$\lambda_i \leftarrow \mathrm{computeDensityConstraintMultiplier}(\mathbf{n}_i)$  \\
$\Delta \mathbf{x}_i\leftarrow \mathrm{solveDensityConstraint}(\lambda_i)$  \\
$\Delta_{u,i}, \Delta_{p,i} \leftarrow \mathrm{solveSuctionDisplacements}(\mathbf{x}_e)$ \\
$\mathbf{x}_i^* = \mathbf{x}_i^* + \Delta \mathbf{x}_i + \mathbf{\hat{y}} \Delta_{u,i} + \Delta_{p,i}$ \\
$\mathbf{x}_i^* \leftarrow \mathrm{computeBoundaryCollision}(\mathbf{x}_i^*)$  \\
% }
% }
}
% \Comment{update step} \\
$\mathbf{x}_i =  \mathbf{x}_i^* $  \Comment{{\scriptsize update position}} \\
$\mathbf{v}_i = \left( \mathbf{x}_i^* - \mathbf{x}_i \right)/\Delta t$ \Comment{{\scriptsize update velocity}} \\
% \For{particle $i \in N$}{
% update velocity $v_{i} = \frac{1}{\Delta t}\left(x_{i}^{t+1}-x_{i}^{t}\right)$
% }
\caption{PBF simulation loop for particles and suction nozzle at positions $\mathbf{x}_i$ and $\mathbf{x}_e$ respectively}
\label{alg:basic_PBF}
\end{algorithm} 



At a high level, our method of incorporating fluid dynamics into autonomous suction control involves three main components: (a) a differentiable fluid model, (b) a suction model between fluid and a suction tool, and (c) a model-predictive controller. The key insights to making the overall autonomous suction work well is that, first, we make the fluid model differentiable by viewing its operations as computational graphs and using back-propagation; then, we make the suction model continuous and differentiable force field that removes particles from the simulation. This allows the entire fluid and suction modeling to be incorporated with the robot manipulator model as a complete, differentiable system of equations that a MPC scheme can effectively and efficiently solve.

\subsection{Differentiable position-based fluid simulation}

% \begin{algorithm}
% \caption{Basic PBF simulation loop}
% \label{alg:basic_PBF}

% \begin{algorithmic}[1]

% \FORALL{particles $i$}
%     \STATE apply external forces $V_i \leftarrow V_i + \Delta t f_{ext}(X_i)$
%     \STATE predict position $X_i^* \leftarrow X_i + \Delta t V_i$
% \ENDFOR

% \FORALL{particles $i$}
%     \STATE find neighboring particles $N_i(X_i^*)$
% \ENDFOR

% \WHILE{iter $<$ solveIterations}

%     \FOR{\textbf{all} particles $i$}
%         \STATE calculate density constraint multiplier $\lambda_i$ using neighbor information
%     \ENDFOR
    
%     \FORALL{particles $i$}
%         \STATE calculate position correction $\Delta P_i$
%         \STATE perform collision detection
%     \ENDFOR
    
%     \FORALL{particles $i$}
%         \STATE update position $X_i^* \leftarrow X_i^* + \Delta P_i$
%     \ENDFOR
    
% \ENDWHILE

% \FORALL{particles $i$}
%     \STATE update velocity $V_i \leftarrow \frac{1}{\Delta t} (X_i^* - X_i)$
%     \STATE update position $X_i \leftarrow X_i^*$
% \ENDFOR

% \end{algorithmic}
% \end{algorithm}
Position-based fluids (PBF) is used as the basis of the fluid simulation because it has good stability even when using large timesteps \cite{macklin2013position}. In the PBF problem, we consider fluids to be  represented by a set of $N$ particles in 3D Cartesian space, $\mathbf{X}\in \mathbb{R}^{3\times N}$. Each particle has position $\mathbf{x}_i \in \mathbb{R}^3$ and velocity $\mathbf{v}_i \in \mathbb{R}^3$. To model fluid physics, these particles are given position-based constraints. In PBF, a density constraint acts on the particle and its neighbors such that they maintain a proximity with one another that as-closely-as-possible matches the resting density of the fluid.
The PBF simulation loop is outlined in Algorithm \ref{alg:basic_PBF}.

% This is the same coordinate system as in the original PBF paper, and it is commonly used in the field of computer graphics. 
% We use position-based fluids (PBF) \cite{macklin2013position} as the basis of our fluid simulation. 
% The PBF solver uses a Lagrangian representation of fluid, which views the fluid as consisting of many particles. 
% The basic simulation loop of PBF is outlined in Algorithm \ref{alg:basic_PBF}.

In order to make this simulation differentiable, all mathematical operations applied to these particles are treated as computation graphs.
From the graph, a gradient back-propagation is used between each operation of the solver. Using this technique, we greatly simplify the application of the chain-rule for complicated operations because the gradient of each step can be computed independently using cached intermediate results. 
% The final end-to-end gradient from the loss to the particle positions by can be obtained by chaining together the .

% \textcolor{red}{ \underline{need to be replaced!}
% As a simple example, consider the input $x=2$ for the operations $y(x)=x^2$ and $z(y)=y^3$. The gradients for the operations are $y'(x)=2x$ and $z'(y)=3y^2$. In the forward pass, we compute $z=64$ and store the intermediate results $x=2$ and $y=4$. In the backward pass, we first use the stored value of $y$ to the gradient of $z$ with respect to $y$ as
% \begin{equation}
%     \frac{dz}{dy}(y=4) = 3\times4^2 = 48
% \end{equation}
% then back-propagate one step to obtain the gradient of $z$ with respect to $x$ as
% \begin{equation}
% \begin{aligned}
%     \frac{dz}{dx}(x=2) & = \frac{dz}{dy}(y=4) \times \frac{dy}{dx}(x=2) \\
%     & = 48\times2\times2 = 192
% \end{aligned}
% \end{equation}
% }

As an example, consider the series of operations in Step 6 of Algorithm \ref{alg:basic_PBF} which computes particle position offsets to satisfy the fluid density constraint.
The formula for computing the correction is given in \cite{macklin2013position} as
% As an example, we consider the series of operations to compute position corrections for each particle, which adjusts the particle positions in order to satisfy the fluid density constraints after all external forces have been applied. This corresponds to step 6 of Algorithm \ref{alg:basic_PBF} and the formula for computing the correction is given in \cite{macklin2013position} as
\begin{equation}
    \Delta \mathbf{x}_i = \frac{1}{\rho_0} \sum_j (\lambda
    _i + \lambda_j + s_{corr}) \nabla W(\mathbf{x}_i - \mathbf{x}_j, h)
    \label{eq:fluid_density_constraint}
\end{equation}
where $\rho_0$ is the rest density of the fluid, $\lambda$ is the density constraint multiplier for each particle $i = 1...M$, $s_{corr}$ is an artificial pressure term used to maintain surface tension, $\nabla W$ is the gradient of the Spiky kernel, given as 
\begin{equation}
    \nabla W (\mathbf{r}, h) = \frac{45}{\pi h^6} (h-||\mathbf{r}||_2)^2 \frac{\mathbf{r}}{||\mathbf{r}||_2}
\end{equation}
and $h$ is the neighborhood radius, which is a parameter of the simulation.
% The computational graph representing this series of operations is shown in Figure \ref{fig:compute_position_correction_graph}.
The computational graph representing these operations is shown in Figure \ref{fig:compute_position_correction_graph}. Because the values of $\lambda$ are also functions of the particle positions from Step 5 in Algorithm \ref{alg:basic_PBF}, the total gradient of $\Delta \mathbf{x}_i$ has contributions from multiple paths: through $S_{corr}$, through $\lambda$, and through $\nabla W$. With the back-propagation view, gradients through each of these paths can be computed independently using cached intermediate values and subsequently combined to obtain the end-to-end gradient.

% , and there is a clear path where the gradients from $\Delta \mathbf{X}_i$ go back to the particle positions through $S_{corr}$.
% Note that the values of $\lambda$ are also functions of the particle positions from Step 5 in Algorithm \ref{alg:basic_PBF}. Therefore the gradient with respect to the particle positions will have contribution


% With the back-propagation view, the gradients simply flow back to $\lambda$ and $\nabla W$, and let their respective gradient subroutines handle gradients going upstream.

\begin{figure}[t]
    \centering
    \vspace{1.8mm}
    \includegraphics[trim=0cm 1cm 0cm 0.5cm, clip, width=0.47\textwidth]{figures/compute_position_correction.pdf}
    \caption{An example computation graph corresponding to (\ref{eq:fluid_density_constraint}). The graph represents the operations for computing the position correction, $ \Delta \mathbf{x}_i $, to satisfy the fluid density constraints.}
    \label{fig:compute_position_correction_graph}
\end{figure}

% From the computational graph, we see a clear path where the gradients $\frac{d L}{d \Delta \mathbf{x}_i}$ go back to the particle positions through $S_{corr}$. However, the values of $\lambda$ and $\nabla W$ are also functions of the particle positions, computed in a previous step. %This make gradient implementation difficult if done in one single step. 
% With the back-propagation view, we can simply let the gradients flow back to $\lambda$ and $\nabla W$, and let their respective gradient subroutines handle gradients going upstream. Using this technique, we greatly simplify the application of the chain-rule for complicated operations because we can independently compute the gradient of each step using cached intermediate results, then obtain the final end-to-end gradient with a series of multiplications. 
%This is particularly useful in computing gradients for our PBF fluid simulation, in which the gradients for a particular particle comes from interactions with all of its neighbors, coupled through many different operations. 

% In our experiments, all forward and backward operations are implemented with the Taichi programming language \cite{hu2019taichi}, which is a Python package for high-performance computation. 

\subsection{Suction model}

% In a real surgical scenario, the suction force is typically very strong and can quickly remove the fluid around the suction nozzle when the suction pump is engaged. 

% A simple way of modeling suction is to remove fluid particles that are within some distance from the nozzle, as the suction force can quickly remove the fluid around the nozzle. However, this formulation is not differentiable. We instead consider suction as a continuous and differnetiable force field that pulls nearby particles towards the nozzle and adds large vertical displacement to the particles within some effective suction area.
The suction force from the surgical tool is modelled as a continuous and differentiable force field that pulls nearby particles towards the nozzle of the tool and adds large vertical displacement to the particles within some effective suction area. Note that we define $y$ as the vertical direction while the $x \text{-} z$ plane represents the horizontal plane. 
% The force field should be a continuous function that is differentiable for all points in space. It should be strongest at the location of the end effector and sharply fall off as distance from the nozzle increases. 
% Using this field, particles near the suction nozzle is quickly moved upwards to a dummy location, and no longer interact with the rest of the particles, effectively removing them from the simulation. 
% Mathematically, the suction field is formulated as follows:
%
The upward displacement field is in the vertical direction, as this is the typical orientation of a suction tool attacking pooling blood. It is modelled after a 2D-Gaussian probability density function (PDF) over the $x\text{-}z$ plane due to its differentiable properties. The magnitude of the upward displacement field experienced by particle $i$ is proportional to the value of the PDF at $([\mathbf{x}_{i}]_x,[\mathbf{x}_{i}]_z)$. 
For a particle $i$ with position $\mathbf{x}_i$, and a suction nozzle at position $\mathbf{x}_e \in \mathbb{R}^3$, the upward displacement, $\Delta_u$, is computed as:
\begin{equation}
% \begin{split}
%     % & [\Delta_{upward}]_x  = 0 \\
% % \end{equation}
% % \begin{equation}
%     % & [\Delta_{upward}]_z   = 0\\
% % \end{equation}
% % \begin{multline}
%     & [\Delta_{upward}]_z = \frac{\mathcal{K}}{\sqrt{\left[(2 \pi)^2 \sigma_x^2 \sigma_z^2\right]}} \cdot \\
%     & ~~~~ \text{exp} \left[- \frac{1}{2} \left( ([\mathbf{x}_{p}]_x-[\mathbf{x}_{e}]_x)^2 \sigma_x^{-2} + ([\mathbf{x}_{p}]_z-[\mathbf{x}_{e}]_z)^2 \sigma_z^{-2} \right) \right]
% % \end{multline}
% \end{split}
\Delta_{u,i} = \mathcal{K} \cdot \frac{\text{exp} \left( -\frac{\left([\mathbf{x}_{i}]_x-[\mathbf{x}_{e}]_x \right)^2}{2\sigma_x^{2}}   - \frac{\left([\mathbf{x}_{i}]_z-[\mathbf{x}_{e}]_z \right)^2}{2\sigma_z^{2}}   \right) }{\sqrt{(2 \pi)^2 \sigma_x^2 \sigma_z^2}}
\end{equation}
where $[\cdot]_x$, $[ \cdot]_y$, and $[ \cdot ]_z$ are the $x,y,z$ coordinates of the position vectors and $\sigma_x$ and $\sigma_z$ are the standard deviations of the 2D Gaussian PDF. The standard deviation controls how narrow the suction region is. Finally, $\mathcal{K} > 0$ controls the size of the upward displacement and is adjusted to control the strength of the suction.
% which is chosen as a large value such that the particles are moved away from the rest of the fluid within 1-2 simulation timesteps.
For the field that pulls particles towards the end-effector at position $\mathbf{x}_e$, the $i$-th particle will experience a displacement given by
\begin{equation}
    \Delta_{p,i} = \frac{\mathbf{x}_{e} - \mathbf{x}_{i}}{||\mathbf{x}_{e} - \mathbf{x}_{i}||_2} \cdot \frac{1}{||\mathbf{x}_{e} - \mathbf{x}_{i}||_2^2 + d}
\end{equation}
where $d$ is a constant that limits the maximum displacement when the particle is very close to the center of the end-effector as well as to avoid division by 0. 
% Furthermore, a sigmoid function, specifically the logistic function, is used to smoothly approximate the boundary of the suction area. 
Finally, the upward field and the field that pulls particles towards the end-effector are summed and added to the particle positions along with the PBF solver corrections as shown in line 7 of Algorithm \ref{alg:basic_PBF}, where $\mathbf{\hat{y}}$ is a normalized vector that describes the direction of upward displacement in the simulation.
This formulation of suction, embedded in a completely differentiable fluid model, enables efficient and stable calculation of gradients from the particle states to the suction tool position. 
% \begin{equation}
%     \mathbf{x}_i^* \Leftarrow \mathbf{x}_i^* + \Delta \mathbf{x}_i + \mathbf{n} \Delta_{u,i} + \Delta_{p,i}
% \end{equation}

\begin{algorithm}[t]
\SetAlgoLined

$\mathbf{X}_{t} \leftarrow \{\mathbf{x}_{1,t}, ~ \mathbf{x}_{2,t}, \cdots\}$ \Comment{{\scriptsize get particle positions}} \\
$\mathbf{V}_{t} \leftarrow \{\mathbf{v}_{1,t}, ~ \mathbf{v}_{2,t}, \cdots\}$ \Comment{{\scriptsize get particle velocities}} \\
$\mathcal{U} = \{\mathbf{x}_{e,t}, ..., \mathbf{x}_{e,h}\} \leftarrow \mathbf{x}_{e,t+h-1}^*$ \Comment{{\scriptsize Initialize trajectory using previous end-effector position}} \\

% \Comment{constraint solving step} \\
% \While{iter $<$ SolverIterations}{
\For{numIterations}{
$\mathrm{initializePBFSimulation}(\mathbf{X}_{t}, \mathbf{V}_{t})$  \Comment{{\scriptsize Setup environment}} \\
$\mathbf{X}_{t+h}, \mathbf{V}_{t+h}\leftarrow \mathrm{runPBFSimulation}(h)$  \Comment{{\scriptsize Run forward PBF for $h$ time-steps}} \\
$ L = \mathrm{computeLoss}(\mathbf{X}_{t+h})$  \Comment{{\scriptsize According to Eq. \ref{eq:loss}}} \\
$ \mathcal{G} = \frac{\partial L}{\partial \mathcal{U}}$  \Comment{{\scriptsize Gradient  back-propagation }} \\
$ \mathcal{U} = \mathcal{U} - \alpha \mathcal{G} $  \Comment{{\scriptsize Gradient descent}}
}
% }

% as in Fig. \ref{fig:compute_position_correction_graph}


% \Comment{update step} \\
$\mathbf{x}_{e,t}^* =  \mathbf{x}_{e,t} $  \Comment{{\scriptsize Optimal MPC control}} \\

% \For{particle $i \in N$}{
% update velocity $v_{i} = \frac{1}{\Delta t}\left(x_{i}^{t+1}-x_{i}^{t}\right)$
% }
\caption{Model predictive end-effector control% at time $t$
}
\label{alg:MPC}
\end{algorithm}


\subsection{Model predictive control formulation}


% To formulate blood suction as a control problem, we consider a non-linear system with dynamics given by the fluid and suction model. The inputs to the system are the positions of the suction end effector, which are our control variables and we denote it as $\mathcal{U}=\{u_t\}$, $u_t \in \mathbf{R}^3$. The outputs of the system are the set of particle positions $\mathbf{X}_t = \{\mathbf{x}_{i,t}\}$, $ \mathbf{x}_{i,t} \in \mathbf{R}^3$, for each particle $i$. 

% The goal of our control algorithm is to remove blood as quickly as possible in order to achieve hemostasis. 
The overall goal of the proposed control problem is to achieve hemostasis as quickly as possible, which corresponds to when all particles in the modelled scene have been lifted from the underlying tissue surfaces of the scene.
This will be formatted as an optimization problem where MPC \cite{camacho2013model} is used to generate a trajectory that the suction nozzle should follow to optimally clear the surgical field from fluids.
Let the control input to the MPC be denoted as $\mathcal{U}=\{\mathbf{x}_{e,t}\}$ where $\mathbf{x}_{e,t}$ is the position of the suction nozzle at time $t$.
The output of the system is the set of particles $\mathbf{X}_t = \{\mathbf{x}_{i,t}\}$.
The MPC is computed over a short horizon, $h$, to find a control trajectory $\{\mathbf{x}_{e,t}^*, ..., \mathbf{x}_{e, t+h}^*\}$ which minimizes the loss over the time frame $[t,t+h]$.
The optimization problem finds the set of control inputs $\mathcal{U}$ that minimizes the loss
\begin{equation}
\label{eq:loss}
\begin{split}
    \min_{\mathcal{U}}   L = \sum_t \sum_i l(\mathbf{x}_{i,t})
\end{split}
\end{equation}
over all timesteps and particles.
The cost function is set to
\begin{equation}
    l(\mathbf{x}_{i,t})= 
    \begin{cases}
        \frac{1}{2} \| y_{goal} - \left[ \mathbf{x}_{i,t} \right]_y \|_2^2, \quad & \text{if $\left[ \mathbf{x}_{i,t} \right]_y < y_{goal}$} \\
        0, \quad & \text{otherwise}
    \end{cases}
\end{equation}
where $y_{goal}$ is a target height set above the surgical cavity. Suction completion is defined as such so that it is continuously differentiable. In MPC, only $\mathbf{x}_{e,t}^*$ is applied to the system, and then another entire horizon length of control is computed again starting at $t+1$.
This routine is detailed in Algorithm \ref{alg:MPC}.

% To optimize the control variables, we utilize model predictive control (MPC). At some time $t$, we consider a short horizon $h$ in the future and find control trajectory $\{\mathbf{x}_t^*, ..., \mathbf{x}_{t+h}^*\}$ to minimize the loss in the time frame $[t,t+h]$. Only $\mathbf{x}_t^*$ is applied to the system. The process is repeated every timestep. The procedure is detailed in Algorithm \ref{alg:MPC}.

% The MPC is computed over a short horizon, $h$, to find a control trajectory $\{\mathbf{x}_{e,t}^*, ..., \mathbf{x}_{e, t+h}^*\}$ which minimizes the loss on the time frame $[t,t+h]$.



To determine a good initial suction point, $\mathbf{x}_{e,0}^*$, a Monte-Carlo approach is utilized.
The process involves sampling many possible starting points from the fluid particle positions, performing roll-outs using the MPC algorithm with these samples over a look-ahead window $m$, and finally selecting the best performing one with regards to removing the most fluid.
An outline is of this procedure is shown in Algorithm \ref{alg:initial}.
% to determine a good initial suction point $u^*_{0}$, i.e. the point where the suction nozzle first interacts with the fluid, which involves sampling many possible starting points, performing roll-outs using the previously discussed MPC algorithm, then selecting the starting point that leads to the best suction performance in some look-ahead window $m$. This procedure is detailed in Algorithm \ref{alg:initial}.

% We use a Monte-Carlo approach to determine a good initial suction point $u^*_{0}$, i.e. the point where the suction nozzle first interacts with the fluid, which involves sampling many possible starting points, performing roll-outs using the previously discussed MPC algorithm, then selecting the starting point that leads to the best suction performance in some look-ahead window $m$. This procedure is detailed in Algorithm \ref{alg:initial}.


% \begin{algorithm}
% \caption{Model predictive end effector control at time $t$}
% \label{alg:MPC}

% \begin{algorithmic}[1]

% \STATE Get particle positions $P_{p,t}$ and velocities $V_{p,t}$

% \STATE Initialize trajectory using previous end effector position $\mathcal{U} = \{u_t, ..., u_{t+H}\} \leftarrow u_{t-1}^*$

% \FOR{numIterations}
%     \STATE Initialize environment with $P_{p,t}$ and $V_{p,t}$
%     \STATE Simulate environment for $H$ timesteps
%     \STATE Compute loss according to Equation \ref{eq:loss}
%     \STATE Compute the gradient $\mathcal{G}$ of loss with respect to $\mathcal{U}$
%     \STATE Perform gradient descent $\mathcal{U} \leftarrow \mathcal{U} - \alpha \mathcal{G}$
% \ENDFOR

% \STATE Select optimal control action $u_t^* = u_t$

% \end{algorithmic}
% \end{algorithm}

% Given that future control actions depend on the current states of the fluid $\mathbf{X}_t$ and the previous end effector position $u^*_{t-1}$, the initial suction point $u^*_{0}$, i.e. the point where the suction nozzle first interacts with the fluid, will have a large effect on the final trajectory and the overall suction performance because it can drastically change the dynamics of the fluid. 
% We use a Monte-Carlo approach to determine a good initial suction point $u^*_{0}$, i.e. the point where the suction nozzle first interacts with the fluid, which involves sampling many possible starting points, performing roll-outs using the previously discussed MPC algorithm, then selecting the starting point that leads to the best suction performance in some look-ahead window $m$. This procedure is detailed in Algorithm \ref{alg:initial}.
\begin{algorithm}[t]
\SetAlgoLined

$\mathbf{X}_{0} \leftarrow \{\mathbf{x}_{1,0}, ~ \mathbf{x}_{2,0}, \cdots\}$ \Comment{ {\scriptsize get particle positions} }\\
$\mathbf{V}_{0} \leftarrow \{\mathbf{v}_{1,0}, ~ \mathbf{v}_{2,0}, \cdots\}$ \Comment{ {\scriptsize get particle velocities} }\\
$\mathbf{S} = \{\mathbf{s}_1, \mathbf{s}_2, \cdots \mathbf{s}_{N}\} \leftarrow \mathbf{X}_{0} $ \Comment{{\scriptsize Uniformly sample $N$ point from $\mathbf{X}_{0}$}} \\

\For{$\mathbf{s}_k$ in $\mathbf{S}$}{
$\mathbf{X}_{t+m}, \mathbf{V}_{t+m}\leftarrow \mathrm{runAlgorithm2}(\mathbf{s}_k, m)$  \Comment{ {\scriptsize Run MPC with $\mathbf{S}$ as initial end-effector position for $m$ time-steps} } \\
$ \mathbf{r}_{k} \leftarrow \lbrace \mathbf{x}_{j,t+m} | \left[ \mathbf{x}_{i,t+m} \right]_y < y_{goal}, \mathbf{x}_{i,t+m} \in \mathbf{X}_{t+m} \rbrace $
\Comment{ {\scriptsize The remaining set of particles not reaching target} } \\
$n_k = \mathrm{card}{(\mathbf{r}_{k})}$
\Comment{ {\scriptsize Number of particles in $\mathbf{r}_{k}$} }
}

$ \mathbf{s}_* \leftarrow \min_{\mathbf{s}_k \in \mathbf{S}}  n_*$  \Comment{Optimal initial suction point} \\
\caption{Selection of initial suction point% at time $t_0$
}
\label{alg:initial}
\end{algorithm}

% \begin{algorithm}
% \caption{Selection of initial suction point at time $t_0$}
% \label{alg:initial}

% \begin{algorithmic}[1]

% \STATE Get particle positions $P_{p,t_0}$ and velocities $V_{p,t_0}$

% \STATE Uniformly sample $N$ points $P_c=\{P_{c,0}, ... P_{c,N-1}\}$ from $P_{p,t_0}$

% \FORALL{points $P_{c,i}$ in $P_c$}
%     \STATE Run Algorithm \ref{alg:MPC} using $P_{c,i}$ as the initial end effector position for $M$ timesteps
%     \STATE Record remaining number of fluid particles $r_i$
% \ENDFOR

% \STATE Select initial suction point $u_0^* = P_{c,i^*}$, where $i^* = \text{arg min} \, r_i$

% \end{algorithmic}
% \end{algorithm}

==> MPC Fluid Suction ICRA/sections/related_works.tex <==
Fluid modeling and simulation have been studied extensively for applications in the natural sciences and computer graphics. For example, smoothed-particle hydrodynamics (SPH) is a method originally developed in 1977 for astrophysical applications \cite{gingold1977smoothed} but have now been widely applied in fluid animations \cite{egst.20141034}. Recent advancements in SPH  \cite{solenthaler2009predictive,akinci2013versatile} aim to improve the accuracy and speed of the simulation. Furthermore, SPH can be embedded into a position-based dynamics simulations to create position-based fluids (PBF), which allows for greater stability when using large timesteps \cite{macklin2013position}. However, these methods are only for the forward simulation of fluid, and do not provide gradients. 
% However, none of these works were applied to robotic applications, in particular for surgial robotics. The integration of robotic control with fluid simulation is a still an open and challenging problem. 

More recently, several methods of differentiable fluid models have been developed. For example, in \cite{ummenhofer2019lagrangian}, the authors introduce a Lagrangian fluid simulation using a new type of convolutional neural network.
Deep neural networks have also been used to learn fluid dynamics in \cite{li2018learning}. 
% The particle-based representation enables adaptability to new environments of unknown dynamics, where dynamic interaction graphs for accurate forward prediction can be obtained within a few observations. The authors show that by using gradient-based optimization, the differentiable simulation can enable different robotic manipulation tasks involving interaction with diverse types of objects.
Schenck and Fox implement PBF using novel fluid dynamic operators to interface with neural networks layers \cite{schenck2018spnets}. 
% The parameters of the network are the fluid parameters natively (e.g., viscosity, cohesion, etc.). This work is particularly interesting because the authors show how to leverage the differentiable network to learn fluid parameters, and perform liquid control and manipulation tasks. However, the PBF dynamics is approximated using network layers, which differs from the analytical model. There might be model mismatch when considering real world fluid. This is clearly demonstrated in the paper when the performance greatly improves with additional perception.
All of these methods provide naturally differentiable fluid models and are capable of optimizing downstream tasks through their gradients.
In this work, we use a similar approach to computing the gradients as \cite{schenck2018spnets} with an extension to differentiable modelling for surgical suction.
Combining the differentiable modelling with MPC allows for the initial blood clearing task of hemostatis to be solved efficiently. 

% All of the above methods provide naturally differentiable fluid models because they use neural network layers. Furthermore, \cite{li2018learning} and \cite{schenck2018spnets} demonstrated that gradients from differentiable simulation can be used for model-based controls in tasks involving robotic interaction with fluids, with better performance and sample efficiency compared to reinforcement learning approaches. However, these methods utilize learned fluid models or approximations that are different from an analytical model. Thus, they may not be able to generalize to different scenarios in real robotic applications. Furthermore, the scenes tested in the simulator are less complex compared to real surgical robotic scenarios. %In particular, none of above papers deal with blood fluid simulation and autonomous suction control. In this paper, we use PBF to model blood fluid dynamics and calculate gradients using back-propagation for model-predictive control (MPC) to tackle the problem of fluid suction.

% More recently, the Taichi programming language \cite{hu2019taichi} can perform automatic differentiation for mathematical operations written under its framework \cite{hu2019difftaichi}. However, the automatic differentiation functions are restrictive, which forces the user to change the implementation of the fluid model in order to obtain gradients. In this work we derive analytical gradients by hand, which is free from the restriction of any framework.

% Crucially, the aforementioned papers have demonstrated that the gradients from differentiable simulations can be used for model-based controls in tasks involving robotic interaction with fluids, with better performance and sample efficiency compared to reinforcement learning approaches. 
% However, most of the proposed papers use deep neural networks to provide the differentiability for inverse control. Thus, it may not be able to generalize to different scenarios in real robotic applications since the fluid model is learned through training data. This can be a challenge in a surgical context. Meanwhile, the scenes tested in the simulator is less complex compared to real surgical robotic scenarios. In particular, none of above papers deal with blood fluid simulation and autonomous suction control. In this paper, we use PBF to model blood fluid dynamics, and calculate gradients using back-propagation for model-predictive control (MPC) to tackle the problem of fluid suction.

==> MPC Fluid Suction ICRA/sections/results.tex <==
\subsection{Simulated suction experiments}

% \begin{figure}
%     \centering
%     \begin{subfigure}{0.235\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/sim_suction_plot_case1.pdf}
%         \label{fig:sim_suction_curve_case1}
%     \end{subfigure}
%     \begin{subfigure}{0.235\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/sim_suction_plot_case2.pdf}
%         \label{fig:sim_suction_curve_case2}
%     \end{subfigure}
%     \caption{Suction curves for the simulated scenes. The time axis starts at 200 because we have a 200 step warm-up period for filling the cavity, which is the same for all methods. \textbf{Left:} In \textit{case 1}, both our method and the end-to-emit trajectory can reach an equilibrium where the cavity is mostly clear, with out method being much faster. \textbf{Right:} In \textit{case 2}, since the scene is nearly symmetrical, the left and right versions of policies are not significantly different. Meanwhile, our method can clear the cavity just as fast as suctioning at the emission point.}
%     \label{fig:sim_suction_curves}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.47\textwidth]{figures/sim_suction_curve_cavity1.png}
%     \caption{Suction curves for \textit{case 1}. The time axis starts at 200 because we have a 200 step warm-up period for filling the cavity, which is the same for all methods. From this figure, we see that both our method and the end-to-emit trajectory can reach an equilibrium where the cavity is mostly clear. However, our method achieves this much faster.}
%     \label{fig:suction_curve_case1}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.47\textwidth]{figures/sim_suction_curve_cavity2.png}
%     \caption{Suction curves for \textit{case 2}. The time axis starts at 200 because we have a 200 step warm-up period for filling the cavity, which is the same for all methods. From this figure, we see that since the scene is nearly symmetrical, suctioning at the left or right end or starting the trajectory from the left or right end are not significantly different. Meanwhile, our method can clear the cavity just as fast as suctioning at the emission point.}
%     \label{fig:suction_curve_case2}
% \end{figure}

% \begin{figure}
%     \centering
%     \begin{subfigure}{0.232\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/traj_length_heatmap.pdf}
%     \end{subfigure}
%     \begin{subfigure}{0.238\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/traj_tau_60_heatmap.pdf}
%     \end{subfigure}
%     \caption{Performance of our method for different emission points in the cavity. The locations of the tiles represent the location of the emission point, while the colors denote trajectory length in $cm$ (left) and 60\% convergence time in simulation timesteps (right). \textbf{Left:} The trajectories generated by our method is longer then the emission point is near the top left or top right corner of the cavity, shorter when the emission point is near the middle. \textbf{Right:} Longer trajectories are correlated with larger 60\% convergence time, which means suction is slower.}
%     \label{fig:heatmap}
% \end{figure}

% \begin{table}[h]
%     \centering
%     \begin{tabular}{cccccc}
%          \hline
%          & Our & Fixed:  & Fixed:  & Fixed:  & End-to-emit\\
%          & method & emission & end & middle & trajectory\\
%          \hline
%          Final count & 11 & 56 & 129 & 54 & 5 \\ 
%          %AUC & 122.73 & 264.98 & 432.08 & 202.80 & 219.38 \\
%          $\tau_{50\%}$ & 36 & 87 & n/a & 23 & 90 \\
%          $\tau_{90\%}$ & 162 & n/a & n/a & n/a & 255 \\
%          \hline
%     \end{tabular}
%     \caption{Final particle count and convergence time for \textit{case 1}. Final count is measured in number of particles, while the convergence times are measured in simulation time steps. Our method achieves similar final particle count as the end-to-emit trajectory, while having significantly lower convergence time, which shows that our method suctions much faster.}
%     \label{tab:results_case1}
% \end{table}

% \begin{table}[h]
%     \centering
%     \begin{tabular}{ccccc}
%          \hline
%          & Our & Fixed:  & Fixed:  & End-to-emit \\
%          & method & emission & end (avg) & trajectory (avg)\\
%          \hline
%          Final count & 3 & 4 & 130 & 7.5 \\ 
%          %AUC & 76.04 & 82.85 & 424.81 & 185.33 \\
%          $\tau_{50\%}$ & 21 & 18 & n/a & 87.5 \\
%          $\tau_{90\%}$ & 102 & 102 & n/a & 172.5 \\
%          \hline
%     \end{tabular}
%     \caption{Final particle count and convergence time for \textit{case 2}. Final count is measured in number of particles, while the convergence times are measured in simulation time steps. Because the scene is roughly symmetric, we take average of policies that have left and right versions. Here we see that our method, fixed suction at the emission point, and the end-to-emit trajectory can all achieve a very low final particle count. The suction speed of our method is comparable to fixed at emission point, which is the fastest.}
%     \label{tab:results_case2}
% \end{table}

In \textit{case 1}, the blood flows around the obstacle from right to left. A human-intuitive strategy would be to suction against the flow, resembling the end-to-emit trajectory. From the left plot in Figure \ref{fig:sim_suction_curves}, we see that our method and the end-to-emit trajectory both reach an equilibrium where almost no blood remain in the cavity within the simulation time limit. We also see that our method suctions much faster than the end-to-emit trajectory which is shown by the convergence times in Table \ref{tab:results_case1}, where our method achieves significantly lower 50\% and 90\% convergence times compared to the end-to-emit trajectory.

In \textit{case 2}, the blood starts in the middle of the cavity and splits into two directions. A human-intuitive strategy is to stay near the middle to suction the blood from the left, right and the emission point at the same time, which resembles the fixed point suction at the emission point. From the right plot in Figure \ref{fig:sim_suction_curves}, we see that all methods, except for fixed point at the end of path, reach an equilibrium where the cavity is almost completely empty. The end-to-emit trajectories suction much slower compared to fixed at the emission point while our method suctions at a rate close to the fixed at the emission point method. 

% Specifically, fixed at emission point have 50\% and 90\% convergence times of 18 and 102 time steps, respectively, while our method has almost the same 50\% and 90\% convergence times at 21 and 102, respectively.

From these two cases, we see that our method can generate very different trajectories dependent on the location of the emission point. To gain insight into how the trajectory varies as we change the emission location, we test our method on the same cavity with different emission points. The emission points are evenly spaced along the sides of the cavity, with emission directions normal to the walls, pointing inside the cavity. The lengths of the resulting trajectories as well as suction speed measured as the 60\% convergence time are plotted as heatmaps, shown in Figure \ref{fig:heatmap}. From the left plot, we see that in general, for emission points near the middle of the cavity, our method will take very short trajectories, which means it stays near the middle. For emission points near the top left and top right corners of the cavity, our method will follow an end-to-emit type path, with a longer trajectory length. From the right plot, we see the intuitive result where longer trajectories typically lead to larger 60\% convergence time, which means suction is slower. 

\subsection{Trajectory validation}

% \begin{figure*}[t]
%     \centering

%     \begin{subfigure}{0.105\textwidth}
% 	\includegraphics[width=1.0\textwidth]{figures/case1_ours/sim_case1_our_trajectory.pdf}
% 	\end{subfigure}
%     \begin{subfigure}{0.16\textwidth}
% 	\includegraphics[width=1.0\textwidth]{figures/case1_ours/render_102.pdf}
% 	\end{subfigure}
%     \begin{subfigure}{0.16\textwidth}
% 	\includegraphics[width=1.0\textwidth]{figures/case1_ours/render_146.pdf}
% 	\end{subfigure}
% 	\begin{subfigure}{0.16\textwidth}
% 	\includegraphics[width=1.0\textwidth]{figures/case1_ours/render_173.pdf}
% 	\end{subfigure}
% 	\begin{subfigure}{0.16\textwidth}
% 	\includegraphics[width=1.0\textwidth]{figures/case1_ours/render_200.pdf}
% 	\end{subfigure} 
% 	\begin{subfigure}{0.16\textwidth}
% 	\includegraphics[width=1.0\textwidth]{figures/case1_ours/render_399.pdf}
% 	\end{subfigure}
	
% 	\vspace{-0.5mm}
	
% 	\begin{subfigure}{0.105\textwidth}
% 	\includegraphics[width=1.0\textwidth]{figures/case1_ours/real_case1_our_trajectory.pdf}
% 	\end{subfigure}
% 	\begin{subfigure}{0.16\textwidth}
% 	\includegraphics[width=1.0\textwidth]{figures/case1_ours/image-018-crop.jpeg}
% 	\end{subfigure}
%     \begin{subfigure}{0.16\textwidth}
% 	\includegraphics[width=1.0\textwidth]{figures/case1_ours/image-020-crop.jpeg}
% 	\end{subfigure}
% 	\begin{subfigure}{0.16\textwidth}
% 	\includegraphics[width=1.0\textwidth]{figures/case1_ours/image-022-crop.jpeg}
% 	\end{subfigure}
% 	\begin{subfigure}{0.16\textwidth}
% 	\includegraphics[width=1.0\textwidth]{figures/case1_ours/image-026-crop.jpeg}
% 	\end{subfigure} 
% 	\begin{subfigure}{0.16\textwidth}
% 	\includegraphics[width=1.0\textwidth]{figures/case1_ours/image-042-crop.jpeg}
% 	\end{subfigure}
	
%     \caption{Comparison between the simulated scene (top) and experiments with the real cavity (bottom) for \textit{case 1} using a trajectory generated from our method. The first image in each row shows the trajectory followed by the tool, with the green arrow denoting the blood emission point. In the simulation, our trajectory can reach an equilibrium where the cavity is almost completely clear. While the trajectory followed by the suction tool closely matches our simulation, due to factors such as surface tension and adhesion, a thin layer of blood remains at the end of the real experiment.}
%     \label{fig:case1_sim_real_comparison}
    
% \end{figure*}

% \begin{figure}
%     \centering
%     \begin{subfigure}{0.47\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/real_suction_plot_case1.pdf}
%     \end{subfigure}
%     \vspace{-2mm}
%     \begin{subfigure}{0.47\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/real_suction_plot_case2.pdf}
%     \end{subfigure}
%     \caption{Suction curves for experiments with silicon rubber cavity. We analyze the curves by splitting them into 4 distinct stages: $(a)$ system initialization; $(b)$ early stage; $(c)$ middle stage; $(d)$ end stage. The top plot corresponds to experiments for \textit{case 1}, and the bottom plot corresponds to experiments for \textit{case 2}.}
%     \label{fig:real_suction_curve}
% \end{figure}



The suction curves for experiments with the silicone rubber cavity are shown in Figure \ref{fig:real_suction_curve}. We analyze the suction curves by roughly splitting each trial into 4 distinct stages. They are labeled on the curves as $(a)$ system initialization, where the tool is moving to initial position without suctioning; $(b)$ early stage, where suction and injection begin; $(c)$ middle stage, where suction and injection are engaged for some time; $(d)$ end stage, where suction and injection are engaged for a long time as the tool reaches the end of the trajectory.

In stage $(a)$, since there is no suction, the behavior is the same across all trials for all suction policies. 

In stage $(b)$, the amount of blood increases as suction starts for some policies. This means the rate of suction is slower than the rate of blood injection. We find that for suction policies that have an initial increase of remaining blood, the suction tool is at the top left or top right corner of the cavity during stage $(b)$, while policies that do not see this behavior start in the middle of the cavity. 

In stage $(c)$, suction and injection reaches an equilibrium where the percentage of remaining blood decreases at a steady rate. In this state, the percentage reaches similar rates of decrease for different suction policies within the same case.

In stage $(d)$, most of the blood in the cavity has been cleared. The remaining blood in the cavity is typically in a thin layer, which causes the effects of surface tension and adhesion to be more pronounced. An example for \textit{case 1} is shown in Figure \ref{fig:case1_sim_real_comparison}. In the simulation, the blood particles can flow without sticking to the face of the cavity, while a patch of blood is stuck in the left half of the cavity in the real experiment due to surface adhesion. Thus, it might be necessary to back track to previously suctioned areas in order to completely clear the cavity, though in practice such little remaining fluid is generally ignored.

We find that the trajectories generated with our method typically start in the middle area of the cavity, which leads to good behaviors in the early stage where the percentage of remaining blood does not increase beyond the initial value. This also helps to reduce the duration of the early stage, which means faster suction compared to other policies. Finally, our trajectories also lead to a low percentage of remaining blood in the end stage.



==> sections/results.tex <==
\subsection{Simulated suction experiments}

% \begin{figure}
%     \centering
%     \begin{subfigure}{0.235\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/sim_suction_plot_case1.pdf}
%         \label{fig:sim_suction_curve_case1}
%     \end{subfigure}
%     \begin{subfigure}{0.235\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/sim_suction_plot_case2.pdf}
%         \label{fig:sim_suction_curve_case2}
%     \end{subfigure}
%     \caption{Suction curves for the simulated scenes. The time axis starts at 200 because we have a 200 step warm-up period for filling the cavity, which is the same for all methods. \textbf{Left:} In \textit{case 1}, both our method and the end-to-emit trajectory can reach an equilibrium where the cavity is mostly clear, with out method being much faster. \textbf{Right:} In \textit{case 2}, since the scene is nearly symmetrical, the left and right versions of policies are not significantly different. Meanwhile, our method can clear the cavity just as fast as suctioning at the emission point.}
%     \label{fig:sim_suction_curves}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.47\textwidth]{figures/sim_suction_curve_cavity1.png}
%     \caption{Suction curves for \textit{case 1}. The time axis starts at 200 because we have a 200 step warm-up period for filling the cavity, which is the same for all methods. From this figure, we see that both our method and the end-to-emit trajectory can reach an equilibrium where the cavity is mostly clear. However, our method achieves this much faster.}
%     \label{fig:suction_curve_case1}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.47\textwidth]{figures/sim_suction_curve_cavity2.png}
%     \caption{Suction curves for \textit{case 2}. The time axis starts at 200 because we have a 200 step warm-up period for filling the cavity, which is the same for all methods. From this figure, we see that since the scene is nearly symmetrical, suctioning at the left or right end or starting the trajectory from the left or right end are not significantly different. Meanwhile, our method can clear the cavity just as fast as suctioning at the emission point.}
%     \label{fig:suction_curve_case2}
% \end{figure}

% \begin{figure}
%     \centering
%     \begin{subfigure}{0.232\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/traj_length_heatmap.pdf}
%     \end{subfigure}
%     \begin{subfigure}{0.238\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/traj_tau_60_heatmap.pdf}
%     \end{subfigure}
%     \caption{Performance of our method for different emission points in the cavity. The locations of the tiles represent the location of the emission point, while the colors denote trajectory length in $cm$ (left) and 60\% convergence time in simulation timesteps (right). \textbf{Left:} The trajectories generated by our method is longer then the emission point is near the top left or top right corner of the cavity, shorter when the emission point is near the middle. \textbf{Right:} Longer trajectories are correlated with larger 60\% convergence time, which means suction is slower.}
%     \label{fig:heatmap}
% \end{figure}

% \begin{table}[h]
%     \centering
%     \begin{tabular}{cccccc}
%          \hline
%          & Our & Fixed:  & Fixed:  & Fixed:  & End-to-emit\\
%          & method & emission & end & middle & trajectory\\
%          \hline
%          Final count & 11 & 56 & 129 & 54 & 5 \\ 
%          %AUC & 122.73 & 264.98 & 432.08 & 202.80 & 219.38 \\
%          $\tau_{50\%}$ & 36 & 87 & n/a & 23 & 90 \\
%          $\tau_{90\%}$ & 162 & n/a & n/a & n/a & 255 \\
%          \hline
%     \end{tabular}
%     \caption{Final particle count and convergence time for \textit{case 1}. Final count is measured in number of particles, while the convergence times are measured in simulation time steps. Our method achieves similar final particle count as the end-to-emit trajectory, while having significantly lower convergence time, which shows that our method suctions much faster.}
%     \label{tab:results_case1}
% \end{table}

% \begin{table}[h]
%     \centering
%     \begin{tabular}{ccccc}
%          \hline
%          & Our & Fixed:  & Fixed:  & End-to-emit \\
%          & method & emission & end (avg) & trajectory (avg)\\
%          \hline
%          Final count & 3 & 4 & 130 & 7.5 \\ 
%          %AUC & 76.04 & 82.85 & 424.81 & 185.33 \\
%          $\tau_{50\%}$ & 21 & 18 & n/a & 87.5 \\
%          $\tau_{90\%}$ & 102 & 102 & n/a & 172.5 \\
%          \hline
%     \end{tabular}
%     \caption{Final particle count and convergence time for \textit{case 2}. Final count is measured in number of particles, while the convergence times are measured in simulation time steps. Because the scene is roughly symmetric, we take average of policies that have left and right versions. Here we see that our method, fixed suction at the emission point, and the end-to-emit trajectory can all achieve a very low final particle count. The suction speed of our method is comparable to fixed at emission point, which is the fastest.}
%     \label{tab:results_case2}
% \end{table}

In \textit{case 1}, the blood flows around the obstacle from right to left. A human-intuitive strategy would be to suction against the flow, resembling the end-to-emit trajectory. From the left plot in Figure \ref{fig:sim_suction_curves}, we see that our method and the end-to-emit trajectory both reach an equilibrium where almost no blood remain in the cavity within the simulation time limit. We also see that our method suctions much faster than the end-to-emit trajectory which is shown by the convergence times in Table \ref{tab:results_case1}, where our method achieves significantly lower 50\% and 90\% convergence times compared to the end-to-emit trajectory.

In \textit{case 2}, the blood starts in the middle of the cavity and splits into two directions. A human-intuitive strategy is to stay near the middle to suction the blood from the left, right and the emission point at the same time, which resembles the fixed point suction at the emission point. From the right plot in Figure \ref{fig:sim_suction_curves}, we see that all methods, except for fixed point at the end of path, reach an equilibrium where the cavity is almost completely empty. The end-to-emit trajectories suction much slower compared to fixed at the emission point while our method suctions at a rate close to the fixed at the emission point method. 

% Specifically, fixed at emission point have 50\% and 90\% convergence times of 18 and 102 time steps, respectively, while our method has almost the same 50\% and 90\% convergence times at 21 and 102, respectively.

From these two cases, we see that our method can generate very different trajectories dependent on the location of the emission point. To gain insight into how the trajectory varies as we change the emission location, we test our method on the same cavity with different emission points. The emission points are evenly spaced along the sides of the cavity, with emission directions normal to the walls, pointing inside the cavity. The lengths of the resulting trajectories as well as suction speed measured as the 60\% convergence time are plotted as heatmaps, shown in Figure \ref{fig:heatmap}. From the left plot, we see that in general, for emission points near the middle of the cavity, our method will take very short trajectories, which means it stays near the middle. For emission points near the top left and top right corners of the cavity, our method will follow an end-to-emit type path, with a longer trajectory length. From the right plot, we see the intuitive result where longer trajectories typically lead to larger 60\% convergence time, which means suction is slower. 

\subsection{Trajectory validation}

% \begin{figure*}[t]
%     \centering

%     \begin{subfigure}{0.105\textwidth}
% 	\includegraphics[width=1.0\textwidth]{figures/case1_ours/sim_case1_our_trajectory.pdf}
% 	\end{subfigure}
%     \begin{subfigure}{0.16\textwidth}
% 	\includegraphics[width=1.0\textwidth]{figures/case1_ours/render_102.pdf}
% 	\end{subfigure}
%     \begin{subfigure}{0.16\textwidth}
% 	\includegraphics[width=1.0\textwidth]{figures/case1_ours/render_146.pdf}
% 	\end{subfigure}
% 	\begin{subfigure}{0.16\textwidth}
% 	\includegraphics[width=1.0\textwidth]{figures/case1_ours/render_173.pdf}
% 	\end{subfigure}
% 	\begin{subfigure}{0.16\textwidth}
% 	\includegraphics[width=1.0\textwidth]{figures/case1_ours/render_200.pdf}
% 	\end{subfigure} 
% 	\begin{subfigure}{0.16\textwidth}
% 	\includegraphics[width=1.0\textwidth]{figures/case1_ours/render_399.pdf}
% 	\end{subfigure}
	
% 	\vspace{-0.5mm}
	
% 	\begin{subfigure}{0.105\textwidth}
% 	\includegraphics[width=1.0\textwidth]{figures/case1_ours/real_case1_our_trajectory.pdf}
% 	\end{subfigure}
% 	\begin{subfigure}{0.16\textwidth}
% 	\includegraphics[width=1.0\textwidth]{figures/case1_ours/image-018-crop.jpeg}
% 	\end{subfigure}
%     \begin{subfigure}{0.16\textwidth}
% 	\includegraphics[width=1.0\textwidth]{figures/case1_ours/image-020-crop.jpeg}
% 	\end{subfigure}
% 	\begin{subfigure}{0.16\textwidth}
% 	\includegraphics[width=1.0\textwidth]{figures/case1_ours/image-022-crop.jpeg}
% 	\end{subfigure}
% 	\begin{subfigure}{0.16\textwidth}
% 	\includegraphics[width=1.0\textwidth]{figures/case1_ours/image-026-crop.jpeg}
% 	\end{subfigure} 
% 	\begin{subfigure}{0.16\textwidth}
% 	\includegraphics[width=1.0\textwidth]{figures/case1_ours/image-042-crop.jpeg}
% 	\end{subfigure}
	
%     \caption{Comparison between the simulated scene (top) and experiments with the real cavity (bottom) for \textit{case 1} using a trajectory generated from our method. The first image in each row shows the trajectory followed by the tool, with the green arrow denoting the blood emission point. In the simulation, our trajectory can reach an equilibrium where the cavity is almost completely clear. While the trajectory followed by the suction tool closely matches our simulation, due to factors such as surface tension and adhesion, a thin layer of blood remains at the end of the real experiment.}
%     \label{fig:case1_sim_real_comparison}
    
% \end{figure*}

% \begin{figure}
%     \centering
%     \begin{subfigure}{0.47\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/real_suction_plot_case1.pdf}
%     \end{subfigure}
%     \vspace{-2mm}
%     \begin{subfigure}{0.47\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/real_suction_plot_case2.pdf}
%     \end{subfigure}
%     \caption{Suction curves for experiments with silicon rubber cavity. We analyze the curves by splitting them into 4 distinct stages: $(a)$ system initialization; $(b)$ early stage; $(c)$ middle stage; $(d)$ end stage. The top plot corresponds to experiments for \textit{case 1}, and the bottom plot corresponds to experiments for \textit{case 2}.}
%     \label{fig:real_suction_curve}
% \end{figure}



The suction curves for experiments with the silicone rubber cavity are shown in Figure \ref{fig:real_suction_curve}. We analyze the suction curves by roughly splitting each trial into 4 distinct stages. They are labeled on the curves as $(a)$ system initialization, where the tool is moving to initial position without suctioning; $(b)$ early stage, where suction and injection begin; $(c)$ middle stage, where suction and injection are engaged for some time; $(d)$ end stage, where suction and injection are engaged for a long time as the tool reaches the end of the trajectory.

In stage $(a)$, since there is no suction, the behavior is the same across all trials for all suction policies. 

In stage $(b)$, the amount of blood increases as suction starts for some policies. This means the rate of suction is slower than the rate of blood injection. We find that for suction policies that have an initial increase of remaining blood, the suction tool is at the top left or top right corner of the cavity during stage $(b)$, while policies that do not see this behavior start in the middle of the cavity. 

In stage $(c)$, suction and injection reaches an equilibrium where the percentage of remaining blood decreases at a steady rate. In this state, the percentage reaches similar rates of decrease for different suction policies within the same case.

In stage $(d)$, most of the blood in the cavity has been cleared. The remaining blood in the cavity is typically in a thin layer, which causes the effects of surface tension and adhesion to be more pronounced. An example for \textit{case 1} is shown in Figure \ref{fig:case1_sim_real_comparison}. In the simulation, the blood particles can flow without sticking to the face of the cavity, while a patch of blood is stuck in the left half of the cavity in the real experiment due to surface adhesion. Thus, it might be necessary to back track to previously suctioned areas in order to completely clear the cavity, though in practice such little remaining fluid is generally ignored.

We find that the trajectories generated with our method typically start in the middle area of the cavity, which leads to good behaviors in the early stage where the percentage of remaining blood does not increase beyond the initial value. This also helps to reduce the duration of the early stage, which means faster suction compared to other policies. Finally, our trajectories also lead to a low percentage of remaining blood in the end stage.


